IN-Flow: Instance Normalization Flow for Non-stationary Time Series Forecasting

Due to the non-stationarity of time series, the distribution shift problem largely hinders the performance of time series forecasting. Existing solutions either rely on using certain statistics to specify the shift, or developing specific mechanisms for certain network architectures. However, the former would fail for the unknown shift beyond simple statistics, while the latter has limited compatibility on different forecasting models. To overcome these problems, we first propose a decoupled formulation for time series forecasting, with no reliance on fixed statistics and no restriction on forecasting architectures. This formulation regards the removing-shift procedure as a special transformation between a raw distribution and a desired target distribution and separates it from the forecasting. Such a formulation is further formalized into a bi-level optimization problem, to enable the joint learning of the transformation (outer loop) and forecasting (inner loop). Moreover, the special requirements of expressiveness and bi-direction for the transformation motivate us to propose instance normalization flow (IN-Flow), a novel invertible network for time series transformation. Different from the classic "normalizing flow" models, IN-Flow does not aim for normalizing input to the prior distribution (e.g., Gaussian distribution) for generation, but creatively transforms time series distribution by stacking normalization layers and flow-based invertible networks, which is thus named "normalization" flow. Finally, we have conducted extensive experiments on both synthetic data and real-world data, which demonstrate the superiority of our method.

==> 2_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

\begin{figure*}[!t]
\centering
\includegraphics[width=0.8\linewidth]{figs/inflow_overview.pdf}
\vspace{-2mm}
\caption{The proposed decoupled formulation (Section \ref{sec:method_formu}) with bi-level optimization (Section \ref{sec:method_optim}) for time series forecasting.} \label{fig:framework_overview}
%\vspace{-2mm}
\end{figure*}

\subsection{Time Series Forecasting} 

Let $\bm{s} = [ \bm{s}_1; \bm{s}_2; \cdots; \bm{s}_T ] \in \mathbb{R}^{T \times D}$ be regularly sampled multi-variate time series with $T$ timestamps and $D$ variates, where $\bm{s}_t \in \mathbb{R}^D$ denotes the multi-variate values at timestamp $t$.
Besides, we use $\bm{x}^L_t \in \mathbb{R}^{L \times D}$ to denote a length-$L$ segment of $\bm{s}$ ending at timestamp $t$ (exclusive), namely $\bm{x}^L_t = \bm{s}_{t-L:t} = [\bm{s}_{t-L}; \bm{s}_{t-L+1}; \cdots; \bm{s}_{t-1}]$.
Similarly, we represent a length-$H$ segment of $\bm{s}$ starting from timestamp $t$ (inclusive) as $\bm{y}^H_t$, so we have $\bm{y}^H_t = \bm{s}_{t:t+H} = [\bm{s}_{t}; \bm{s}_{t+1}; \cdots; \bm{s}_{t+H-1}]$.
The classic time series forecasting formulation is to project
historical observations $\bm{x}^L_t$ into their subsequent future values ${\bm{y}}^H_t$.
Specifically, a typical forecasting model $f_\theta : \mathbb{R}^{L \times D} \to \mathbb{R}^{H \times D}$ produces forecasts by $\hat{\bm{y}}^H_t = f_\theta( \bm{x}^H_t )$ where $\hat{\bm{y}}^H_t$ stands for the forecasting result, $\theta$ encapsulates the model parameters, and $H$ and $L$ are usually referred to as the lengths of horizon (lookahead) windows and lookback windows, respectively.


\subsection{Bi-level Optimization}
\label{sec:bg_bilevel_optim}
Bi-level optimization problems are one kind of optimization problems in which a set of variables in an objective function are constrained by the optimal solution of another optimization problem \cite{colson2007overview}. Specifically, given two functions $J_{in}$ and $J_{out}$ as the inner objectives and outer objectives, we consider two set of variables $\theta \in \mathbb{R}^m, \phi \in \mathbb{R}^n$ as the inner variables and outer variables, respectively; the bi-level problem can be given by
$\underset{\phi, \theta_\phi}{\min} J_{out}(\theta_\phi,\phi)$ such that $\theta_\phi \in \arg \underset{\theta}{\min} J_{in}(\theta, \phi) $.
Bi-level problems have involved in many applications, including hyperparmeter optimization, multi-task, meta-learning, etc  \cite{colson2007overview,sinha2017review,franceschi2018bilevel,pu2023dynamic,pu2023pami}.



\subsection{Normalzing Flows} 
\label{sec:bg_flows}
Normalzing flows \cite{papamakarios2021normalizing}, as one common kind of invertible neural networks, can conduct transformation between distributions. Given a high-dimensional random variable $\mathbf{x} \in \mathcal{X}$, flow-based models \cite{dinh2014nice,dinh2016density,papamakarios2017masked,kingma2018glow} transform densities $p_{\mathcal{X}}$ into certain target distribution $p_{\mathcal{Z}}$ (e.g., an isotropic Gaussian) on a latent variable $\mathbf{z} \in \mathcal{Z}$. The transformation is a bijection $g: \mathcal{X} \to \mathcal{Z}$ (with inverse $ g^{-1}$). 
The probability density can be written by the change of variable formula as:
% \begin{equation}
%     p_{\mathcal{X}}(\mathbf{x}) = p_{\mathcal{Z}}(\mathbf{z}) \left|\operatorname{det} \left( \frac{\partial g(\mathbf{x})}{\partial \mathbf{x}} \right) \right|
% \end{equation}
$p_{\mathcal{X}}(\mathbf{x}) = p_{\mathcal{Z}}(\mathbf{z}) \left|\operatorname{det} \left( \frac{\partial g(\mathbf{x})}{\partial \mathbf{x}} \right) \right|$
where $\partial g(\mathbf{x}) / \partial \mathbf{x}$ is the Jacobian of $g$ at $\mathbf{x}$. The transformation $g$ is composed of a sequence of differentiable invertible (or bijective) mapping functions $g = g_1 \circ g_2 \circ \cdots \circ g_P$ that map 
$\mathbf{x} \stackrel{g_1}{\longleftrightarrow} \mathbf{h}_1 \stackrel{g_2}{\longleftrightarrow}  \mathbf{h}_2 \cdots \stackrel{g_P}{\longleftrightarrow} \mathbf{z}$ reversibly.  
% Usually, flow-based models are trained via maximum likelihood on training data. Thus, the probability density function of the flows given a data point is
% $\log p_{\mathcal{X}}(\mathbf{x}) = \log p_{\mathcal{Z}}(\mathbf{z}) + \log \left|\operatorname{det} \left( \frac{\partial \mathbf{z}}{\partial \mathbf{x}} \right) \right| =\log p_{\mathcal{Z}}(\mathbf{z})+\sum_{i=1}^P  
% \log \left| \operatorname{det}\left( \partial \mathbf{h}_i / \partial \mathbf{h}_{i-1} \right) \right|$, where  $\mathbf{h}_0 \triangleq \mathbf{x}$ and $\mathbf{h}_P \triangleq \mathbf{z}$; $\log \left| \operatorname{det}\left( \partial \mathbf{h}_i / \partial \mathbf{h}_{i-1} \right) \right|$ is called log-determinant of $\left( \partial \mathbf{h}_i / \partial \mathbf{h}_{i-1} \right)$. The key idea of designing transformation in normalizing flows is to make the computation of log-determinant simple and easy \cite{kobyzev2020normalizing,papamakarios2021normalizing}.





\iffalse
Under the change of variables formula, the probability density function (PDF) of the flow given a data point can be written as:
\begin{equation}
\begin{aligned}
\log p_{\mathcal{X}}(\mathbf{x}) &= \log p_{\mathcal{Z}}(\mathbf{z}) + \log \left|\operatorname{det} \left( \frac{\partial \mathbf{z}}{\partial \mathbf{x}} \right) \right| \\
&=\log p_{\mathcal{Z}}(\mathbf{z})+\sum_{i=1}^P  
\log \left| \operatorname{det}\left( \partial \mathbf{h}_i / \partial \mathbf{h}_{i-1} \right) \right|
\end{aligned}
\end{equation}
where we let $\mathbf{h}_0 \triangleq \mathbf{x}$ and $\mathbf{h}_P \triangleq \mathbf{z}$; $\log \left| \operatorname{det}\left( \partial \mathbf{h}_i / \partial \mathbf{h}_{i-1} \right) \right|$ is called log-determinant, the logarithm of the absolute value of the determinant of the Jacobian matrix $\left( \partial \mathbf{h}_i / \partial \mathbf{h}_{i-1} \right)$. The key idea of designing transformation in normalizing flows is to make the computation of log-determinant simple and easy \cite{kobyzev2020normalizing,papamakarios2021normalizing}.
\fi






==> 3_method.tex <==

\section{Methodology}
\label{sec:method}

In this section, we elaborate on our principled approach that makes no assumption to specify distribution shifts and accommodates all kinds of forecasting models.
% First, we introduce a decoupled formulation that separates distribution transformation and forecasting functionalities in Section \ref{sec:method_formu}; 
% then, we formalize a bi-level optimization problem to enable joint learning of two sides in Section \ref{sec:method_optim}, and present our specifically designed IN-Flow model in Sections~\ref{sec:method_in_flow}.
% Besides, Figure \ref{fig:framework_overview} demonstrates an overview of our framework.
% short version
First, we introduce a decoupled formulation in Section \ref{sec:method_formu}; 
then, we formalize a bi-level optimization problem for the decoupled formulation in Section \ref{sec:method_optim}, and present our specifically designed IN-Flow model in Sections~\ref{sec:method_in_flow}.
Besides, Figure \ref{fig:framework_overview} demonstrates an overview of our framework.



\subsection{A Decoupled Formulation}
\label{sec:method_formu}

It is noteworthy that the aforementioned formulation ($\hat{\bm{y}}^H_t = f_{\theta} ( \bm{x}^H_t )$),
embracing a large body of forecasting models~\cite{Oreshkin2020N-BEATS,zhou2021informer,wu2021autoformer,minhao2022SCINet,zeng2022D-linear},
essentially follows a \emph{stationary} assumption:
\emph{the conditional data probability $P(\bm{y}^H_t | \bm{x}^L_t)$ does not change over time}.
However in practice, some recent studies~\cite{kim2022RevIN,du2021ada,liu2022NonstatTranformers} have well recognized the wide existence of non-stationary properties in real-world time series.
Besides, we further note that those distribution shift patterns can be far more sophisticated than simple statistical measures, such as mean and standard deviation used in~\cite{kim2022RevIN}.
Thus arbitrarily specifying non-stationary properties has the risk of removing certain information crucial to forecasting and is limited in tackling more diverse distribution shifts.


To provide a generic approach to address the problem of distribution shift in time-series forecasting, we regard the procedure of removing non-stationary information as a special distribution transformation (\textit{transformation module}) and separate its functionality from the \textit{forecasting module}.
Accordingly, we develop a decoupled formulation as:
\begin{equation}
    p(\bm{y}^H_t | \bm{x}^L_t) = 
    p(\bm{y}^H_t | \tilde{\bm{y}}^H_t) \cdot 
    p(\tilde{\bm{y}}^H_t | \tilde{\bm{x}}^L_t)  \cdot 
    p(\tilde{\bm{x}}^L_t | \bm{x}^L_t)
    \label{eq:decouple_formula}
\end{equation}
where $\tilde{\bm{x}}^L_t$ and $\tilde{\bm{y}}^H_t$ denote the transformed variables of $\bm{x}^L_t$ and $\bm{y}^H_t$, respectively.
We assume that $\tilde{\bm{x}}^L_t$ and $\tilde{\bm{y}}^H_t$ come from certain desired distributions with shifted information removed but forecasting-related information preserved.
In this way, we decouple the modeling of conditional data distribution $p(\bm{y}^H_t | \bm{x}^L_t)$ into three parts:
(i) $p(\tilde{\bm{x}}^L_t | \bm{x}^L_t)$, performing a transformation on raw input series to remove non-stationary (shifted) information;
(ii) $p(\tilde{\bm{y}}^H_t | \tilde{\bm{x}}^L_t)$, conducting forecasting on the transformed space;
(iii) $p(\bm{y}^H_t | \tilde{\bm{y}}^H_t)$, performing a reverse transformation to recover certain non-stationary patterns and produce final forecasts.

This decoupled formulation lays the foundation for respective parameterization and optimization of transformation and forecasting modules.
Then in addition to the forecasting function $f_\theta$, we introduce another two functions to be responsible for the bi-directional distribution transformations in the transformation module.
To be specific, $g_{\phi^L}: \bm{x}^L_t \rightarrow \tilde{\bm{x}}^L_t$,  parameterized by $\phi^L$, stands for the transformation from a raw data distribution $\mathcal{X}^L$ to a desired distribution $\tilde{\mathcal{X}}^L$ without non-stationary information, and $g^{-1}_{\phi^H}: \bm{x}^H_t \rightarrow \tilde{\bm{x}}^H_t$ parameterized by $\phi^H$ denotes the reverse transformation from $\tilde{\mathcal{X}}^H$ to $\mathcal{X}^H$.
Accordingly, we emit a forecast $\hat{\bm{y}}^H_t$ given an input $\bm{x}^L_t$ as:
\begin{align}
    \hat{\bm{y}}^H_t = g^{-1}_{\phi^H} \left(
        f_\theta \left( g_{\phi^L} \left( \bm{x}^L_t \right)
        \right)
    \right)
    \label{eq:decouple_forecast}
\end{align}



\subsection{A Bi-level Optimization Problem}
\label{sec:method_optim}

Given the decoupled formulation, we further consider a learning procedure to fulfill the needs of 1) removing distribution shifts that hinder the forecasting performance and 2) performing accurate forecasting based on samples from a transformed stationary distribution.
Motivated by these two-sided objectives, we naturally develop a \textit{bi-level optimization} problem~\cite{colson2007overview}:
\begin{equation}
\begin{aligned}
\phi_* & = \underset{\phi}{\arg \min}\; \mathcal{L} \left( \theta_*(\phi), \phi, \mathcal{T}_{val} \right) \\
\operatorname{s.t.} \quad \theta_*(\phi) &= \underset{\theta}{\arg \min}\; \mathcal{L} \left( \theta, \phi, \mathcal{T}_{train} \right)
\end{aligned}
\label{eq:bilevel_optim}
\end{equation}
where $\phi$ encapsulates $\phi^H$ and $\phi^L$,
$\mathcal{T}_{train}$ and $\mathcal{T}_{val}$ denote the sets of time steps in training and validation periods, respectively,
and $\mathcal{L}(\theta, \phi, \mathcal{T}) = \sum_{t \in \mathcal{T}} \ell ( \bm{y}^H_t, g^{-1}_{\phi^H} ( f_\theta ( g_{\phi^L} (\bm{x}^L_t) ) ) )$ is the summation of losses, specified by $\ell (\bm{y}^H_t, \hat{\bm{y}}^H_t)$, over all time steps in $\mathcal{T}$.
The inner loop optimization indicates that given any transformation model parameterized by $\phi$, the solution $\theta_*(\phi)$ minimizes the forecasting losses on the training data, which ensures the effective learning of the forecasting module on the transformed space.
The outer loop optimization aims to identify the transformation solution $\phi_*$ that contributes to the best generalization performance on the validation data, which aligns with our motivation to remove uncertain shifted information hindering forecasting.

Moreover, a standard approach to solve the bi-level optimization problem of Equation (\ref{eq:bilevel_optim}) is to introduce hyper gradients~\cite{chen2022gradient}.
Nevertheless, the calculation of hyper gradients involves the computation of $\frac{\partial \mathcal{L}(\theta_*(\phi), \phi, \mathcal{T}_{val})}{\partial \theta_*(\phi)} \frac{\partial \theta_*(\phi)}{\partial \phi}^T$, which can be prohibitive when performing exact inner optimization.
Therefore, we adopt the first-order approximation, as did in \cite{liu2018darts}, to cut off the gradient dependency introduced by $\frac{\partial \theta_*(\phi)}{\partial \phi}$ and alternate between the following two gradient updates:
\begin{equation}
\begin{aligned}
    \theta_{i+1} &= \theta_i - \alpha \frac{\partial \mathcal{L}(\theta_i, \phi_i, \mathcal{T}_{train})}{\partial \theta_i}, \\
    \phi_{i+1} &= \phi_i - \gamma \frac{\partial \mathcal{L}(\theta_{i+1}, \phi_i, \mathcal{T}_{val})}{\partial \phi_i}.
\end{aligned}
\end{equation}
where $i$ means the $i$-th iteration; $\alpha$ and $\gamma$ are the learning rate for the forecasting module and the transformation module respectively.
In this way, we actually turn the original bi-level optimization into alternate optimization \cite{chen2022gradient}.
While in practice, we find that applying such an approximation to our case brings very fast computation with negligible performance compromise.




\subsection{Instance Normalizaiton Flow}
\label{sec:method_in_flow}


Though the decoupled formulation with bi-level optimization can accommodate any $f_\theta$, another critical challenge is the design of the transformation module and optimization for $\phi$.
First, the module should have adequate ability to transform data distributions effectively (expressiveness).
Second, the module is responsible for the bi-directional transformation between $\mathcal{X}$ (${\mathcal{X}}^L, {\mathcal{X}}^H$) and $\tilde{\mathcal{X}}$ ($\tilde{\mathcal{X}}^L, \tilde{\mathcal{X}}^H$). Such considerations inspire us to leverage the key idea of \textit{normalizing flows} \cite{kobyzev2020normalizing}, one kind of invertible networks \cite{ardizzone2018analyzing} that transform data distributions.

\begin{figure}[!t]
\centering
\subfigure[RealNVP]{
\includegraphics[width=0.33\linewidth]{figs/real.pdf}
%\caption{fig1}
}
\hspace{-0mm}
\subfigure[IN-Flow]{
\includegraphics[width=0.35\linewidth]{figs/inflow.pdf}
}
\vspace{-2mm}
\caption{The specific architecture of RealNVP \cite{dinh2016density} and our IN-Flow. We discuss the difference of pre-norm and post-norm in Section \ref{sec:exp_ablation} and take the pre-norm version as IN-Flow.}
\label{fig:method_inflow}
\vspace{-3mm}
\end{figure}

Existing normalizing flows conduct reversible transformation on one raw data distribution (see Section \ref{sec:bg_flows}). In contrast, we notice our formulation is composed of two transformations, $g_{\phi^L}: \bm{x}_t^L \rightarrow \tilde{\bm{x}}_t^L$ and $g_{\phi^H}^{-1}: \tilde{\bm{x}}_t^H \rightarrow \bm{x}_t^H$, which actually operate in two variable spaces ($g_{\phi^L}$ on $\mathcal{X}^L \in \mathbb{R}^{L \times D}$ and $g_{\phi^H}$ on $\mathcal{X}^H \in \mathbb{R}^{H \times D}$), due to the difference of lookback length ($L$) and horizon length ($H$). 
Nonetheless, these two distributions, $p_{\mathcal{X}^L}(\bm{x}^L)$ and $p_{\mathcal{X}^H}(\bm{x}^H)$, undoubtedly share many common parts in distribution because their samples are generated by segmenting the same time series ($\bm{s}$).
Therefore, to fulfill bi-directional transformations on two variable spaces and capture the common patterns between them, we develop a novel invertible neural architecture, namely \textit{instance normalization flow} (IN-Flow), that instantiates $g_{\phi^L}$ and $g_{\phi^H}$ as a single network and works on variable length of time series, also referred to as $g_{\phi}$ for brevity.


Flow-based models \cite{dinh2014nice,dinh2016density,papamakarios2017masked,kingma2018glow} usually adopt batch normalization in their architectures for a stable training. However, a batch in time series forecasting may consist of samples of various distributions due to distribution shift~\cite{kim2022RevIN}. In such cases, batch normalization could meet with instability in calculating batch statistics and influence the transformation \cite{shen2020powernorm}. Moreover, we notice instance normalization has recently been effective in computer vision \cite{ulyanov2016instance,huang2017arbitrary} and can be an alternative to get over the instability \cite{dumoulin2016learned}. And in the domain of time series, the sequence format can make distribution shift relieved with the application of instance normalization~\cite{kim2022RevIN}.
Inspired by them, our IN-Flow includes instance normalization layer which is written given $d$-th variate by:
\begin{equation}
    {\bm{h}'}^{L,(d)}_{t} = 
    \left( \bm{h}_{t}^{L,(d)}- \mathbf{\mu}_{t}^{(d)} \right)
    {\left( \sigma^{2(d)}_{t} +\epsilon \right)}^{-\frac{1}{2}}
    \operatorname{exp}(\gamma^{(d)}_t)
    + \beta_t^{(d)}
\label{eq:instance_norm_forward}
\end{equation}
where ${\bm{h}'}_t^{L,(d)}$ are the corresponding mappings of $\bm{h}_{t}^{L,(d)} \in \mathbb{R}^{L\times1}$. Supposing it's the first layer of $g_\phi$, we have $\bm{h}_{t}^{L,(d)} \triangleq \bm{x}_{t}^{L,(d)}$, 
$\mu_{t}^{(d)} = \frac{1}{L} \sum \bm{x}_{t}^{L,(d)} = \frac{1}{L} \sum_{t-L}^{t-1} s_t^{(d)}$ as the instance mean, $\sigma^{2(d)}_{t} = \frac{1}{L} \sum_{t-L}^{t-1} \left( {s}_{t}^{(d)} - \mu_t^{(d)} \right)^2$ as square of instance std.. %, with ${s}_{t}^{(d)}$ as the value of $d$-th variate at timestamp $t$. 
And $\gamma_t^{(d)}$, $\beta_t^{(d)}$ are affine parameters for transformation. We leave more details in Appendix \ref{sec:appendix_inflow_design}.





In addition, to make the transformation more expressive, we follow  previous works to include 
one common reversible design of flows, \textit{affine coupling layers} \cite{dinh2014nice,dinh2016density} as part of IN-Flow. In implementation, we let coupling layers work on the feature (variate) dimension by:
% \begin{equation}
% \left\{\begin{array}{l}
% \bm{h}_{t}^{L, (1:d_c)}=\bm{x}_{t}^{L,(1:d_c)}  \\
% \bm{h}_{t}^{L,(d_c:D)} = \bm{x}_{t}^{L,(d_c:D)} \odot  s \left( \bm{x}_{t}^{L,(1:d_c)} \right)  + 
%   t\left( \bm{x}_{t}^{L,(1:d_c)} \right)
% \end{array}\right.
% \label{eq:method_coupling_layer}
% \end{equation}
\begin{equation}
\left\{\begin{array}{l}
{\bm{h}'}_{t}^{L, (1:d_c)}=\bm{h}_{t}^{L,(1:d_c)}  \\
{\bm{h}'}_{t}^{L,(d_c:D)} = \bm{h}_{t}^{L,(d_c:D)} \odot  s \left( \bm{h}_{t}^{L,(1:d_c)} \right)  + 
  t\left( \bm{h}_{t}^{L,(1:d_c)} \right)
\end{array}\right.
\label{eq:method_coupling_layer}
\end{equation}
where usually we let $d_c = \lceil \frac{D}{2} \rceil$ stand for the split position; $\bm{h}_{t}^{L,(1:d_c)} \in \mathbb{R}^{L \times d_c}$ denotes data composed of first $d_c$ variates of $\bm{h}_{t}^{L}$ and $\bm{h}_{t}^{L,(d_c:D)} \in \mathbb{R}^{L \times (D-d_c)}$ denotes the left $D-d_c$ variates; $s$ and $t$ are scale and translation functions mapping from $\mathbb{R}^{d_c}$ to $\mathbb{R}^{D-d_c}$; ${\bm{h}'}_{t}^{L}$ is the processed output.



Overall, the main architecture of IN-Flow is by stacking \textit{instance normalization} and \textit{coupling layers} iteratively, similar to other classic normalizing flows such as RealNVP \cite{dinh2016density}, as shown in Figure \ref{fig:method_inflow}.
We also adopt \textit{Split} and \textit{Permute} operations \cite{dinh2014nice,dinh2016density,kingma2018glow}
to assist for stacking layers. 
Note that both Equation (\ref{eq:instance_norm_forward}) and Equation (\ref{eq:method_coupling_layer}) belong to the transformation of $p(\tilde{\bm{x}}^L_t | \bm{x}^L_t)$. We can also accordingly write the \textit{inverse} transformation of above layers for $p(\bm{y}^H_t | \tilde{\bm{y}}^H_t)$ in IN-Flow. %We leave details of inverse transformation in Appendix \ref{sec:appendix_inflow_design}.


















==> 4_experiments.tex <==
\section{Experiments}
\label{sec:experiment}
Our empirical studies aim to answer the questions: 
1) With some solutions existing, why should we further study distribution shift in time series forecasting?  
2) How much benefit can our framework gain for time series forecasting compared with existing state-of-the-art models in real-world settings? 
3) Does each part of {IN-Flow} designs (including optimization) count for good forecasting performance?

\textbf{Baselines.} We mainly consider two kinds of state-of-the-art (SoTA) methods for distribution shift in time series. For the SoTA model-agnostic normalization technique, RevIN \cite{kim2022RevIN}, we adopt one best-performed pure fully-connected network based architecture, N-BEATS \cite{oreshkin2019n} and one representative transformer-based architecture, Autoformer \cite{wu2021autoformer} as two main backbones for comparison.
For the SoTA architecture-specific method, Nonstationary Transformers \cite{liu2022NonstatTranformers}, we take vanilla Transformer \cite{vaswani2017attention}, Informer \cite{zhou2021informer} and Autoformer \cite{wu2021autoformer} as backbones. 
More baseline details are in Appendix \ref{sec:appendix_baseline}.


\textbf{Evaluation Details.}
We evaluate time series forecasting performance on the classic mean squared error (MSE) and mean absolute error (MAE). %To directly reflect distribution shift in time series, all the experiments and evaluations are conducted on original data without data scaling or normalization unless mentioned especially.
The reported metrics on real-world data are scaled for readability. More evaluation details are included in Appendix \ref{sec:appendix_more_real_evaluation_details}.






\subsection{Evaluation on Synthetic Data} \label{sec:exp_synthetic}
To intuitively illustrate the importance of modelling distribution shifts in forecasting and the superiority of IN-Flow, we generate synthetic time series data with distributions shifted. We first group each neighbored $\tau$ points as a segment and let every segment follows one distribution. Supposing to synthesize one series $\{s_1, \cdots, s_T\}$ of length $T$, this series can be regarded to have $U = \lceil T/\tau \rceil$ segments, where the $u$-th segment follows its distribution $\mathcal{P}_u$. 
We can thus control the degree of time series distribution shift through adjusting $\tau$ and $\mathcal{P}_u$. Under such settings, both $p(\bm{x}_t^{L})$ and $p( \bm{y}^{H}_t|\bm{x}_t^{L})$ keep shifted over time if lookback length $L>\tau$ and lookahead length $H>\tau$. Then for each $\mathcal{P}_u$, we simply make a regular cosine wave signal to model simple periodic patterns in time series. Specifically, we let $s_t =  A_u \operatorname{cos}(2\pi\frac{1}{T_u} t+B_u) + C_u$ if time index $t$ belongs to $u$-th segment, where $A_u, T_u, B_u, C_u$ indicate amplitude, period, phase and level parameters for the $u$-th segment. %, respectively. After data generation, all the forecasting models have access to the mixed part of $s_t$ for training.

\begin{figure}
    \centering
    % \vspace{-4mm}%
    \includegraphics[width=\linewidth]{expfigs/main_syn.pdf}
    %\vspace{-0.5em}
    \vspace{-4mm}
    \caption{Performance comparison on Synthetic-1 dataset. Full results are included in Appendix \ref{sec:appendix_more_syn_evaluation}.} 
    \label{fig:main_syn_evaluation}
    \vspace{-3mm}
\end{figure}

Following the above rules, we make three synthetic datasets, called Synthetic-1/2/3 by varying different $\tau$ and $\mathcal{P}_u$. 
Due to space limit, we include more details about synthetic datasets in Appendix \ref{sec:appendix_more_syn_generation} and more experiments in Appendix~\ref{sec:appendix_more_syn_evaluation}. 
Figure \ref{fig:main_syn_evaluation} shows two different comparisons of different backbones on Synthetic-1 dataset. We notice that in our simulation settings, both two state-of-the-art techniques RevIN and Nonstationary Transformers would fail significantly, causing about 10\% performance decrease on N-BEATS and 16\% performance decrease on Autoformer. These results clearly demonstrate their limitations in overcoming distribution shifts in forecasting when meeting some severely-shifted time series, while IN-Flow can still improve their forecasting ability.




%\vspace{-2mm}
\subsection{Evaluation on Real-world Data} \label{sec:exp_real_world}
%Apart from simulation experiments on synthetic data, 
Apart from simulation experiments, we further perform experiments on real-world datasets. We adopt six existing shifted datasets following previous forecasting literatures: Electricity transformer temperature datasets %\footnote{\url{https://github.com/zhouhaoyi/ETDataset}} 
include time series of oil temperature and power load collected from electricity transformers in China. \textbf{\textit{ETTm2}} dataset is recorded at a fifteen minutes frequency ranging from July 2016 to July 2018.
In contrast, \textbf{\textit{ETTh1}} dataset and \textbf{\textit{ETTh2}} dataset are in recorded every hour.
\textbf{\textit{Weather}} dataset 
%\footnote{\url{https://www.bgc-jena.mpg.de/wetter/}} 
contains meteorological measurements of 21 weather indicators, which are collected 10-minutely in 2020.
%from the Weather Station of the Max Planck Biogeochemistry Institute in Germany in 2020.
\textbf{\textit{CAISO}} dataset 
%\footnote{\url{http://www.energyonline.com/Data/}} 
includes hourly electricity load series in different zones of California ranging from 2017 to 2020. \textbf{\textit{NordPool}} dataset 
%\footnote{\url{https://www.nordpoolgroup.com}} 
includes hourly energy production volume series of several European countries in 2020. See Appendix \ref{sec:appendix_more_real_data_details} for dataset details.
%For more dataset details, see Appendix XX. 

For a stable evaluation, we perform z-score normalization for each backbone models and inverse the forecasting results to report metrics.
We rerun all the models under four different seeds to report the average MSE/MAE on the testset of each dataset. We mainly follow previous works \cite{zhou2021informer,wu2021autoformer} to split the dataset into train/validation/test data. Notably, we cut the 90\% and 10\% of training data into $\mathcal{T}_{train}$ and  $\mathcal{T}_{val}$.
To cover short/long-term forecasting, we set the length of lookback and horizon window from 48 to 336. We train the forecasting models using L2 loss and Adam \cite{kingma2014adam} optimizer on single NVIDIA A100 40GB GPU. For more implementation details, please see Appendix \ref{sec:appendix_more_real_implementation_details}.

\input{tables/main_exp.tex}

\subsubsection{Main Results}



Figure \ref{table:main_exp} demonstrates the overall performance comparison of the SoTA model-agnostic method, RevIN \cite{kim2022RevIN} with our IN-Flow. Based on the results, we notice that tough RevIN can boost the backbones in some cases, it can also lead to  worse (or comparable) performance, which signifies limitations of RevIN in relying on fixed statistics to handle distribution shifts. 
However, IN-Flow consistently improves backbones models under different settings over different datasets. Notably, with the lookback/horizon length as 48 on Weather dataset, IN-Flow improves Autoformer by 32.6\% ($0.597 \to 0.402$) and improves N-BEATS by 44.6\% ($0.781 \to 0.432$) on MSE. Another case on CAISO dataset is that  the MSE of Autoformer with IN-Flow is reduced from 1.789 to 0.823, which achieves a very large (54.0\%) improvement. The overall superior performance shows great potential of IN-Flow in enhancing deep forecasting models.



We also include performance comparison of IN-Flow in Table \ref{table:main_nonstation} compared with the SoTA architecture-specific method, Non-stationary Transformers \cite{liu2022NonstatTranformers}, in which we consider three transformer-based models as backbones to compose Non-stationary Transformer/Informer/Autoformer. The full results are included in Appendix \ref{sec:appendix_more_real_exp_results}.
From Table \ref{table:main_nonstation}, we easily observe that IN-Flow achieves a significant improvement than Non-stationary Transformers. Especially, on Weather dataset, such an improvement even comes to 43.7\% ($0.389 \to 0.219$) compared with Non-stationary Transformer and 53.4\% ($0.533 \to 0.248$) compared with Non-stationary Autoformer when the prediction length is 168. The superiority signifies that even though IN-Flow is a model-agnostic method, it can have great adaptation for transformer-based models and even beat architecture-specific methods with tailor-designed mechanisms de-stationary attention \cite{liu2022NonstatTranformers}, which shows great potential of its compatibility.

\input{tables/main_nonstaion.tex}

% \begin{figure*}[htbp]
% \centering
% \subfigure[ETTh2 dataset]{
% \includegraphics[width=0.33\linewidth]{expfigs/ETTh2_case.pdf}
% %\caption{fig1}
% }
% \hspace{-4mm}
% \subfigure[ETTm2 dataset]{
% \includegraphics[width=0.33\linewidth]{expfigs/ETTm2_case.pdf}
% %\caption{fig1}
% }
% \hspace{-4mm}
% \subfigure[CAISO dataset]{
% \includegraphics[width=0.33\linewidth]{expfigs/ca_case.pdf}
% %\caption{fig1}
% }
% \caption{Visualizations to intuitively demonstrate the effectiveness of IN-Flow. The raw input series is first transformed into the target distribution with shift information removed but forecasting-related information preserved. Then, the forecasting module performs forecasting and the transformation module recovers the forecasting results from the target distribution to the raw distribution.}
% \end{figure*}


\iffalse
\subsection{Ablation Studies} \label{sec:exp_ablation}

In order to verify the effectiveness of our designs, we conduct adequate ablation studies by adjusting each key component successively.
First, we consider the classic normalizing flows as the transformation module: (i) \textit{RealNVP} \cite{dinh2016density} adopts the coupling layers \cite{dinh2014nice} and the batch normalization \cite{ioffe2015batch}; (ii) \textit{RealNVP-c} \cite{dinh2016density} only adopts the coupling layers for transformation and removes batch normalization. %Note that for above two methods, we adopt the implementation of XXX that ignores the multi-scale architecture \cite{dinh2016density,kingma2018glow}. 
Second, we consider two variants of our IN-Flow: (i) \textit{IN-Flow-J} jointly optimizes the transformation module and the forecasting module on the training data without bi-level optimization; (ii) \textit{IN-Flow-T} changes the relative position of coupling layers (post-norm). %and instance normalization and puts the instance normalization to the {t}ail of flows. %The two variants validate the design of bi-level optimization and IN-Flow architecture, respectively. 
We include more details and visualize these methods in Appendix \ref{sec:appendix_ablation_methods_decription}.



\input{tables/main_ablation.tex}
Table \ref{table:main_brief_ablation} demonstrates the brief results of the ablation studies with N-BEATS as the backbone. 
We include the full results of ablation studies on N-BEATS and Autoformerin Appendix \ref{sec:appendix_ablation_exp_results}. 
From Table \ref{table:main_brief_ablation}, we can easily observe that when the original RealNVP is coupled with forecasting model, the performance is much more worse and cannot even compare with other methods. However, removing batch normalization makes the performance become comparable. This clearly shows batch normalization cannot fit for the transformation module to joint optimize with the forecasting models.
Moreover, when we apply instance normalization instead, the performance (of IN-Flow and its variants) is obviously improved compared with RealNVP series methods.
We notice that IN-Flow can outperform its two variants in most cases, which demonstrates the effectiveness of our designs in the architecture and the optimization.
\fi



% \begin{figure}[thbp]
% \centering
% \subfigure[Training Loss]{
% \includegraphics[width=0.49\linewidth]{expfigs/trainloss.pdf}
% \label{fig:optimization_case_training_loss}
% %\caption{fig1}
% }
% \hspace{-4mm}
% \subfigure[Validation Loss]{
% \includegraphics[width=0.468\linewidth]{expfigs/valloss.pdf}
% \label{fig:optimization_case_validation_loss}
% %\caption{fig1}
% }
% % \vspace{-4mm}
% \caption{Learning loss curves with or without IN-Flow.}
% \vspace{-3mm}
% \end{figure}





\subsection{Additional Experiments} \label{sec:exp_addition}

\subsubsection{Ablation Studies} \label{sec:exp_ablation}

In order to verify the effectiveness of our designs, we conduct adequate ablation studies by adjusting each key component successively.
First, we consider the classic normalizing flows as the transformation module: (i) \textit{RealNVP} \cite{dinh2016density} adopts the coupling layers \cite{dinh2014nice} and the batch normalization \cite{ioffe2015batch}; (ii) \textit{RealNVP-c} \cite{dinh2016density} removes batch normalization from \textit{RealNVP}. %Note that for above two methods, we adopt the implementation of XXX that ignores the multi-scale architecture \cite{dinh2016density,kingma2018glow}. 
Second, we consider two variants of our IN-Flow: (i) \textit{IN-Flow-J} jointly optimizes the transformation module and the forecasting module on the training data without bi-level optimization; (ii) \textit{IN-Flow-T} changes the relative position of coupling layers (post-norm). %and instance normalization and puts the instance normalization to the {t}ail of flows. %The two variants validate the design of bi-level optimization and IN-Flow architecture, respectively. 
We include more details and analysis in Appendix \ref{sec:appendix_ablation_methods_decription}.

% \vspace{-1mm}
\subsubsection{Optimization Process}
\begin{figure}
\centering
\subfigure[Training Loss]{\includegraphics[width=0.48\linewidth]{expfigs/trainloss.pdf}
\label{fig:optimization_case_training_loss}}
\hspace{-2mm}
\subfigure[Validation Loss]{\includegraphics[width=0.468\linewidth]{expfigs/valloss.pdf}
\label{fig:optimization_case_validation_loss}}
\vspace{-3mm}
\caption{Learning loss curves with or without IN-Flow.}
\vspace{-3mm}
\end{figure}
To further study the learning process of IN-Flow, we visualize the learning loss curves of N-BEATS and IN-Flow. Figure \ref{fig:optimization_case_training_loss} and Figure \ref{fig:optimization_case_validation_loss} demonstrate the training loss and validation loss curve on CAISO dataset respectively, 
which correspond to the inner loop and outer loop optimization updates as mentioned in Section \ref{sec:method_optim}. 
We notice that with IN-Flow the training loss of N-BEATS has faster convergence 
which signifies the transformation module improves the learning of forecasting module. After about 50 epochs, though the two training loss curves come close, the validation loss of IN-Flow is far lower than pure N-BEATS, which is attributed to the transformation module that relieves distribution shifts for less validation errors and better generalization in forecasting.




\begin{figure}
\centering
% \vspace{-5mm}
\includegraphics[width=\linewidth]{expfigs/main_case_v4.pdf}
\vspace{-3mm}
\caption{Visualization of decoupled forecasting on \textit{ETTh2} dataset. Input series $\bm{x}_t^L$ (black line) is firstly transformed to $\tilde{\bm{x}}_t^L$ (grey line), performed forecasting to $\tilde{\bm{y}}_t^H$ (light-blue line) and inversely transformed to  ${\bm{y}}_t^H$ (blue line). We include more visualization cases in Appendix \ref{sec:appendix_visualization_cases}.}
\label{fig:visualizaition_cases}
\vspace{-1mm}
\end{figure}



% \vspace{-1mm}
\subsubsection{Visualization Analysis}
To intuitively illustrate the superiority of our decoupled formulation and IN-Flow, we visualize specific forecasting cases. Figure \ref{fig:visualizaition_cases} shows the forecasting process of RevIN and IN-Flow with N-BEATS as the backbone. We visualize the three parts in modelling conditional distribution $p(\bm{y}^H_t | \bm{x}^L_t)$ (see Section \ref{sec:method_formu}) in Figure \ref{fig:visualizaition_cases}: (i) $p(\tilde{\bm{x}}^L_t | \bm{x}^L_t)$: transform input series (from black to grey line); (ii) $p(\tilde{\bm{y}}^H_t | \tilde{\bm{x}}^L_t)$: perform forecasting on transformed space (from grey to light-blue line); (iii) $p(\bm{y}^H_t | \tilde{\bm{y}}^H_t)$: inversely transform for final forecasts (from light-blue to blue line).
We can observe that IN-Flow not only removes distribution shift but also keeps \textit{forecasting-related oscillations}, which result into more meaningful forecasts in the transformed space. Moreover, in the inverse transformation stage, IN-Flow can produce more accurate forecasts recovered from the transformed distribution.
This intuitive case signifies IN-Flow has a more expressive transformation than naive normalization and help forecasting models for more accurate predictions.
We have included more visualization cases and conducted more analysis towards our decoupled forecasting process; see Appendix \ref{sec:appendix_visualization_cases} for details.


==> 5_related_work.tex <==

\section{Related Work}
\subsection{Models for Time Series Forecasting}
Time series forecasting has been a longstanding research topic in various domains~\cite{han2021joint,fan2022feature,fan2023dewp}. At an early stage, researchers have proposed statistical modeling approaches, including exponential smoothing \cite{holt1957forecasting} and auto-regressive moving averages (ARMA) \cite{whittle1963prediction}. With the great successes of deep learning, many deep learning models~\cite{deng2024bigger,yi2023frequency,yi2023survey} have been developed for time series forecasting. 
Some studies have proposed forecasting models using recurrent neural network \cite{rangapuram2018deep, salinas2020deepar, zia2020residual} or convolution neural networks \cite{bai2018empirical,minhao2022SCINet}.
Some others studies have applied pure fully-connected neural network for forecasting \cite{Oreshkin2020N-BEATS,fan2022depts,zeng2022D-linear}. Transformer \cite{vaswani2017attention} has also been used for the time series forecasting task. Many research have improved vanilla transformer
in attention computation, memory consumption, etc, to enhance forecasting \cite{zhou2021informer,wu2021autoformer,zhou2022fedformer}.
% \vspace{-3mm}

\subsection{Distribution Shifts in Time Series}

Time series forecasting suffers from distribution shift issue considering distributions of real-world series change over time \cite{akay2007grey}. 
For this problem, some normalization techniques are proposed: Adaptive Norm \cite{ogasawara2010adaptive} rescale time series through global minimum and maximum; DAIN \cite{passalis2019deep} use adaptive z-score normalization by global average and std. for the task of time series classification. Recently, RevIN \cite{kim2022RevIN} proposes to use instance normalization to reduce time series distribution shift. Most of these works \cite{ogasawara2010adaptive,passalis2019deep,kim2022RevIN,fan2023dish} use statistics to specify the distribution shift and accordingly normalize series, which is limited in expressiveness.
Also, there are some proposed specific mechanisms designed for certain network architectures to relieve the distribution shift: \cite{du2021ada} proposed Adaptive RNNs to handle the shift problem on top of recurrent neural networks (RNNs).
More recently, Nonstationary Transformers \cite{liu2022NonstatTranformers} have proposed series stationarization and de-stationary attention to enhance transformer-based forecasting models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> expfigs/tables/main_ablation.tex <==
% \begin{table}[h]
% \small
% \centering
% % \begin{threeparttable}
% \caption{Ablation studies with taking N-BEATS as the backbone. Evaluations are the average performance of four seeds on MSE. Underlined are the best results. See Appendix \ref{sec:appendix_ablation_exp_results} for full results.
% } \label{table:main_brief_ablation}
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{p{0.01cm} c|   ccccc}
% \toprule
% && {\scriptsize RealNVP} & {\scriptsize RealNVP-c} & {\scriptsize IN-Flow-J} & {\scriptsize IN-Flow-T} & {\scriptsize IN-Flow} \\
% %&& { RealNVP-c} & { RealNVP} & { IN-Flow-J} & { IN-Flow-T} & { IN-Flow} \\
% \midrule
% \multirow{3}{*}{ \rotatebox{90}{\scriptsize ETTh2} }
% &{\scriptsize 48}&13.823&1.380&1.264&1.240& \underline{1.229}\\
% &{\scriptsize 168}&13.493&2.192&1.848&1.772&\underline{1.752}\\
% &{\scriptsize 336}&11.690&2.317&\underline{1.872}&1.961&{1.928}\\
% \midrule
% \multirow{3}{*}{ \rotatebox{90}{\scriptsize ETTm2} }
% &{\scriptsize 48}&12.291&1.031&\underline{0.876}&0.938&{0.894}\\
% &{\scriptsize 168}&14.474&1.530&1.231&1.214&\underline{1.212}\\
% &{\scriptsize 336}&16.525&1.826&1.546&1.567&\underline{1.541}\\
% \midrule
% \multirow{3}{*}{ \rotatebox{90}{\scriptsize Weather} }
% &{\scriptsize 48}&1.039&0.533&0.495&0.460&\underline{0.432}\\
% &{\scriptsize 168}&0.771&0.183&0.186&0.191&\underline{0.182}\\
% &{\scriptsize 336}&0.604&0.190&0.183&0.193&\underline{0.179}\\
% \midrule
% \multirow{3}{*}{ \rotatebox{90}{\scriptsize CAISO} }
% &{\scriptsize 48}&4.355&0.568&0.541&0.516&\underline{0.514}\\
% &{\scriptsize 168}&5.013&{1.126}&\underline{1.054}&1.153&1.150\\
% &{\scriptsize 336}&3.710&1.479&\underline{1.358}&1.535&1.518\\
% \bottomrule
% \end{tabular}
% % }
% % \label{table:ablation}
% % \end{threeparttable}
% \end{table}

% \begin{wrapfigure}{r}{0.65\linewidth}
%     \centering
%     %\vspace{-0.5em}%
%     \includegraphics[width=\linewidth]{expfigs/main_syn.pdf}
%     %\vspace{-0.5em}
%     \vspace{-3mm}
%     \caption{Performance comparison on Synthetic-1 dataset. Full results are included in Appendix \ref{sec:appendix_more_syn_evaluation}.} 
%     \label{fig:main_syn_evaluation}
% \end{wrapfigure}
\begin{wraptable}{r}{0.65\linewidth}
% \begin{table}[h]
\small
\centering
% \begin{threeparttable}
\vspace{-6mm}
\caption{Ablation studies with taking N-BEATS as the backbone. Evaluations are the average performance of four seeds on MSE. Underlined are the best results. See Appendix \ref{sec:appendix_ablation_exp_results} for full results.
} \label{table:main_brief_ablation}
% \resizebox{\linewidth}{!}{
\begin{tabular}{p{0.01cm} c|ccccc}
\toprule
&& {\scriptsize RealNVP} & {\scriptsize RealNVP-c} & {\scriptsize IN-Flow-J} & {\scriptsize IN-Flow-T} & {\scriptsize IN-Flow} \\
%&& { RealNVP-c} & { RealNVP} & { IN-Flow-J} & { IN-Flow-T} & { IN-Flow} \\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize ETTh2} }
&{\scriptsize 48}&13.823&1.380&1.264&1.240& \underline{1.229}\\
&{\scriptsize 168}&13.493&2.192&1.848&1.772&\underline{1.752}\\
&{\scriptsize 336}&11.690&2.317&\underline{1.872}&1.961&{1.928}\\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize ETTm2} }
&{\scriptsize 48}&12.291&1.031&\underline{0.876}&0.938&{0.894}\\
&{\scriptsize 168}&14.474&1.530&1.231&1.214&\underline{1.212}\\
&{\scriptsize 336}&16.525&1.826&1.546&1.567&\underline{1.541}\\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize Weather} }
&{\scriptsize 48}&1.039&0.533&0.495&0.460&\underline{0.432}\\
&{\scriptsize 168}&0.771&0.183&0.186&0.191&\underline{0.182}\\
&{\scriptsize 336}&0.604&0.190&0.183&0.193&\underline{0.179}\\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize CAISO} }
&{\scriptsize 48}&4.355&0.568&0.541&0.516&\underline{0.514}\\
&{\scriptsize 168}&5.013&{1.126}&\underline{1.054}&1.153&1.150\\
&{\scriptsize 336}&3.710&1.479&\underline{1.358}&1.535&1.518\\
\bottomrule
\end{tabular}
% }
% \end{table}
\end{wraptable}




==> expfigs/tables/main_ablation_cr.tex <==

\begin{table}[!t]
\centering
% \begin{threeparttable}
\small

\caption{Ablation studies taking N-BEATS as the backbone.
} \label{table:appendix_ablation_nbeats}
\vspace{-3mm}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|cccccccccc}
\toprule
\multicolumn{2}{c}{Method}& 
\multicolumn{2}{c}{ RealNVP }&\multicolumn{2}{c}{ RealNVP-c}& 
\multicolumn{2}{c}{ IN-Flow-J}&\multicolumn{2}{c}{ IN-Flow-T}& 
\multicolumn{2}{c}{IN-Flow}\\ 
\cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} 
\multicolumn{2}{c}{Metric}&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE&
MSE& MAE\\
\midrule \midrule
% \multirow{4}{*}{ \rotatebox{90}{ETTh1} }
% &48&3.081&3.720&\textbf{0.947}&{1.677}&1.026&1.701&0.969&1.635&0.951&\textbf{1.624}\\
% &96&2.705&3.481&\textbf{1.019}&1.816&1.096&1.840&1.058&1.794&1.027&\textbf{1.768}\\
% &168&2.112&2.981&\textbf{1.123}&1.934&1.141&1.917&1.140&{1.916}&\textbf{1.139}&\textbf{1.914}\\
% &336&2.203&3.109&\textbf{1.116}&2.033&1.170&2.098&1.173&2.053&1.146&2.044\\
% \midrule
% \multirow{4}{*}{ \rotatebox{90}{ETTh2} }
% &48&13.823&9.810&1.380&2.422&1.264&2.220&1.240&2.202&\textbf{1.229}&\textbf{2.182}\\
% &96&15.647&10.350&1.879&2.842&1.533&2.487&{1.530}&{2.479}&\textbf{1.520}&\textbf{2.412}\\
% &168&13.493&9.527&2.192&3.083&1.848&2.719&1.772&2.711&\textbf{1.752}&\textbf{2.681}\\
% &336&11.690&8.658&2.317&3.335&{1.872}&{2.834}&1.961&2.881&1.928&2.847\\
% \midrule
% \multirow{4}{*}{ \rotatebox{90}{ETTm2}}
% &48&12.291&8.917&1.031&2.063&{0.876}&{1.847}&0.938&1.925&0.894&1.866\\
% &96&12.977&9.053&1.175&2.188&{0.971}&{1.918}&0.993&1.933&0.980&1.945\\
% &168&14.474&9.799&1.530&2.467&1.231&2.189&{1.214}&2.164&\textbf{1.212}&\textbf{2.162}\\
% &336&16.525&10.893&1.826&2.744&1.546&2.479&1.567&2.502&\textbf{1.541}&\textbf{2.477}\\
% \midrule
\multirow{4}{*}{ \rotatebox{90}{Weather}}
&48&1.039&4.973&0.533&2.665&0.495&1.840&0.460&1.731&\textbf{0.432}&\textbf{1.698}\\
&96&1.033&5.354&0.225&1.698&0.234&1.365&0.251&1.376&\textbf{0.223}&\textbf{1.328}\\
&168&0.771&4.724&0.183&1.494&0.186&1.303&0.191&1.243&\textbf{0.182}&\textbf{1.217}\\
&336&0.604&4.647&0.190&1.579&0.183&1.416&0.193&1.382&\textbf{0.179}&\textbf{1.311}\\
% \midrule
% \multirow{4}{*}{ \rotatebox{90}{CAISO}}
% &48&4.355&1.412&0.568&0.368&0.541&0.350&0.516&0.345&\textbf{0.514}&\textbf{0.341}\\
% &96&5.311&1.530&0.885&0.441&\textbf{0.777}&\textbf{0.419}&0.906&0.434&0.878&0.428\\
% &168&5.013&1.495&1.126&0.502&\textbf{1.054}&\textbf{0.481}&1.153&0.494&1.150&0.498\\
% &336&3.710&1.213&1.479&0.592&\textbf{1.358}&\textbf{0.571}&1.535&0.607&1.518&0.602\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{NordPool}}
&48&3.137&1.147&1.166&0.643&{1.167}&{0.643}&1.188&0.639&\textbf{1.150}&\textbf{0.632}\\
&96&2.541&1.029&1.602&0.758&1.620&0.759&1.597&0.757&\textbf{1.596}&\textbf{0.756}\\
&168&2.008&0.910&2.006&0.870&1.980&0.845&1.972&0.849&\textbf{1.918}&\textbf{0.836}\\
&336&2.100&0.921&2.283&0.927&{2.152}&{0.898}&2.082&0.880&\textbf{2.098}&\textbf{0.884}\\
% \midrule
\bottomrule
\end{tabular}
}
% \begin{tablenotes}
% \end{tablenotes}
% \end{threeparttable}
\vspace{-0mm}
\end{table}

==> expfigs/tables/main_exp.tex <==
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}
% \fontsize{8.5pt}{9}\selectfont
\small
\caption{Performance comparison of time series forecasting on backbone models and IN-Flow. The length of lookback/horizon windows is prolonged from 48 to 336 to cover short and long forecasting settings.
} \label{table:main_exp}
\vspace{-4mm}
\begin{tabular}{c|c|cccc|cccc|cccc|cccc}
\toprule
\multicolumn{2}{c}{Method}& \multicolumn{2}{c}{PatchTST}&\multicolumn{2}{c}{+{IN-Flow}}& \multicolumn{2}{c}{iTransformer}&\multicolumn{2}{c}{{+IN-Flow{}}}& 
\multicolumn{2}{c}{{Autoformer}}&   \multicolumn{2}{c}{+{IN-Flow}} & \multicolumn{2}{c}{N-BEATS}&\multicolumn{2}{c}{+{IN-Flow}} \\ 
\cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14} \cmidrule(r){15-16} \cmidrule(r){17-18} 
\multicolumn{2}{c}{Metric}&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE\\
\midrule \midrule
\multirow{4}{*}{ \rotatebox{90}{ETTh1} }
&48  & 1.128 & 1.865 & \textbf{0.936} & \textbf{1.635} & 1.051 & 1.717 & \textbf{0.811} & \textbf{1.244} & 1.237 & 2.010  & \textbf{1.215} & \textbf{1.937} & 0.959 & 1.637 & \textbf{0.951} & \textbf{1.624} \\
&96  & 1.320  & 2.109 & \textbf{1.025} & \textbf{1.782} & 1.188 & 1.933 & \textbf{0.896} & \textbf{1.542} & 1.710  & 2.347 & \textbf{1.428} & \textbf{2.141} & 1.072 & 1.789 & \textbf{1.027} & \textbf{1.768} \\
&168 & 2.001 & 2.679 & \textbf{1.077} & \textbf{1.888} & 1.917 & 2.624 & \textbf{0.901} & \textbf{1.925} & 2.139 & 2.739 & \textbf{1.303} & 
\textbf{2.095} & 1.223 & 1.989 & \textbf{1.139} & \textbf{1.914} \\
&336 & 1.784 & 2.613 & \textbf{1.121} & \textbf{2.021} & 1.734 & 2.568 & \textbf{1.107} & \textbf{1.189} & 2.444 & 2.965 & \textbf{1.502} & \textbf{2.305} & 1.222 & 2.083 & \textbf{1.146} & \textbf{2.044} \\
\midrule
\multirow{4}{*}{ \rotatebox{90}{ETTm2} }
&48  & 1.116 & 2.204 & \textbf{0.925} & \textbf{1.908} & 1.094 & 2.168 & \textbf{0.958} & \textbf{1.972} & 1.477 & 2.469 & \textbf{1.459} & \textbf{2.432} & 1.329 & 2.308 & \textbf{1.229} & \textbf{2.182} \\
&96  & 1.503 & 2.699 & \textbf{0.992} & \textbf{1.965} & 1.470 & 2.178 & \textbf{0.996} & \textbf{1.973} & 1.962 & 2.901 & \textbf{1.869} & \textbf{2.748} & 1.628 & 2.604 & \textbf{1.570} & \textbf{2.496} \\
&168 & 1.708 & 2.783 & \textbf{1.213} & \textbf{2.202} & 1.352 & 2.472 & \textbf{1.248} & \textbf{2.275} & 1.898 & 2.919 & \textbf{1.834} & \textbf{2.831} & 2.148 & 3.021 & \textbf{1.752} & \textbf{2.681} \\
&336 & 2.664 & 3.465 & \textbf{1.564} & \textbf{2.482} & 2.124 & 2.713 & \textbf{1.678} & \textbf{2.532} & 2.271 & 3.235 & \textbf{2.113} & \textbf{3.003} & 2.376 & 3.339 & \textbf{1.928} & \textbf{2.847} \\
\midrule
\multirow{4}{*}{ \rotatebox{90}{Electricity}}
&48  & 0.632 & 0.366 & \textbf{0.554} & \textbf{0.342} & 0.513 & 0.319 & \textbf{0.421} & \textbf{0.312} & 0.686 & 0.398 & \textbf{0.592} & \textbf{0.381} & 0.698 & 0.431 & \textbf{0.594} & \textbf{0.422} \\
&96  & 0.882 & 0.698 & \textbf{0.589} & \textbf{0.341} & 0.710 & 0.558 & \textbf{0.479} & \textbf{0.313} & 0.936 & 0.763 & \textbf{0.669} & \textbf{0.397} & 0.912 & 0.751 & \textbf{0.872} & \textbf{0.723} \\
&168 & 1.678 & 0.541 & \textbf{0.882} & \textbf{0.389} & 1.341 & 0.413 & \textbf{0.790} & \textbf{0.329} & 1.989 & 0.576 & \textbf{0.943} & \textbf{0.437} & 2.031 & 0.582 & \textbf{1.521} & \textbf{0.503} \\
&336 & 2.482 & 0.814 & \textbf{2.104} & \textbf{0.768} & 2.012 & 0.654 & \textbf{1.678} & \textbf{0.594} & 2.934 & 0.898 & \textbf{2.521} & \textbf{0.813} & 2.835 & 0.872 & \textbf{2.671} & \textbf{0.852} \\
\midrule
\multirow{4}{*}{ \rotatebox{90}{Weather}}
&48  & 1.003 & 3.291 & \textbf{0.413} & \textbf{1.710} & 1.001 & 3.288 & \textbf{0.447} & \textbf{1.897} & 1.297 & 3.217 & \textbf{0.402} & \textbf{1.844} & 0.981 & 3.226 & \textbf{0.432} & \textbf{1.698} \\
&96  & 0.335 & 1.886 & \textbf{0.279} & \textbf{1.541} & 0.334 & 1.886 & \textbf{0.301} & \textbf{1.629} & 0.658 & 3.327 & \textbf{0.285} & \textbf{1.663} & 0.246 & 1.642 & \textbf{0.223} & \textbf{1.328} \\
&168 & 0.338 & 2.138 & \textbf{0.207} & \textbf{1.421} & 0.337 & 2.138 & \textbf{0.263} & \textbf{1.581} & 0.398 & 2.260 & \textbf{0.253} & \textbf{1.708} & 0.192 & 1.392 & \textbf{0.182} & \textbf{1.217} \\
&336 & 0.385 & 2.375 & \textbf{0.192} & \textbf{1.475} & 0.384 & 2.373 & \textbf{0.228} & \textbf{1.535} & 0.570 & 2.996 & \textbf{0.255} & \textbf{1.712} & 0.194 & 1.520 & \textbf{0.179} & \textbf{1.311} \\
\midrule
\multirow{4}{*}{ \rotatebox{90}{CAISO}}
&48  & 0.986 & 0.499 & \textbf{0.641} & \textbf{0.383} & 0.906 & 0.425 & \textbf{0.627} & \textbf{0.377} & 1.789 & 0.740 & \textbf{0.823} & \textbf{0.467} & 1.099 & 0.684 & \textbf{0.514} & \textbf{0.341} \\
&96  & 0.898 & 0.451 & \textbf{0.828} & \textbf{0.422} & 0.833 & 0.424 & \textbf{0.799} & \textbf{0.393} & 2.428 & 0.826 & \textbf{1.289} & \textbf{0.576} & 0.886 & 0.440 & \textbf{0.878} & \textbf{0.428} \\
&168 & 1.369 & 0.577 & \textbf{1.161} & \textbf{0.500} & 1.297 & 0.503 & \textbf{1.071} & \textbf{0.411} & 2.832 & 0.907 & \textbf{1.344} & \textbf{0.575} & 1.189 & 0.504 & \textbf{1.150} & \textbf{0.498} \\
&336 & 2.541 & 0.852 & \textbf{1.636} & \textbf{0.604} & 2.124 & 0.712 & \textbf{1.524} & \textbf{0.456} & 3.148 & 0.960 & \textbf{1.809} & \textbf{0.679} & 1.612 & 0.607 & \textbf{1.518} & \textbf{0.602} \\
\midrule
\multirow{4}{*}{ \rotatebox{90}{NordPool}}
&48  & 1.304 & 0.664 & \textbf{1.156} & \textbf{0.636} & 1.331 & 0.800 & \textbf{1.233} & \textbf{0.769} & 1.632 & 0.765 & \textbf{1.478} & \textbf{0.732} & 1.192 & 0.639 & \textbf{1.150} & \textbf{0.632} \\
&96  & 1.771 & 0.799 & \textbf{1.687} & \textbf{0.777} & 1.851 & 0.936 & \textbf{1.796} & \textbf{0.823} & 2.187 & 0.889 & \textbf{2.071} & \textbf{0.852} & 1.644 & 0.764 & \textbf{1.596} & \textbf{0.756} \\
&168 & 2.513 & 0.986 & \textbf{2.009} & \textbf{0.865} & 2.597 & 1.035 & \textbf{2.584} & \textbf{0.908} & 2.596 & 0.992 & \textbf{2.430} & \textbf{0.957} & 2.044 & 0.867 & \textbf{1.918} & \textbf{0.836} \\
&336 & 2.946 & 1.040 & \textbf{2.010} & \textbf{0.887} & 3.022 & 0.976 & \textbf{2.138} & \textbf{0.941} & 2.993 & 1.236 & \textbf{2.079} & \textbf{0.887} & 2.557 & 0.953 & \textbf{2.098} & \textbf{0.884} \\
\midrule
\bottomrule
\end{tabular}
\vspace{-0.5mm}
\end{threeparttable}
}
\end{table*}


==> expfigs/tables/main_exp_old.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{threeparttable}
% \fontsize{8.5pt}{9}\selectfont
\small
\caption{Performance comparison of time series forecasting on backbone models (Autoformer and N-BEATS) with z-score-norm, RevIN and IN-Flow. The length of windows is prolonged from 48 to 336 to cover short/long-term forecasting. %The reported metrics are the average results under four seeds (see Appendix \ref{sec:appendix_more_real_evaluation_details}).
%Due to space limit, results of Informer are in Appendix.
} \label{table:main_exp}
\begin{tabular}{c|c|cccccc|cccccc}
\toprule
\multicolumn{2}{c}{Method}& \multicolumn{2}{c}{Autoformer}&\multicolumn{2}{c}{+{RevIN}}& \multicolumn{2}{c|}{+IN-Flow}&\multicolumn{2}{c}{{N-BEATS{$^*$}}}& 
\multicolumn{2}{c}{+{RevIN}}&   \multicolumn{2}{c}{+{IN-Flow}}\\ 
\cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14} 
\multicolumn{2}{c}{Metric}&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE\\
\midrule \midrule
\multirow{4}{*}{ \rotatebox{90}{ETTh1} }
%&24&0.988&1.774&1.161&1.846&\textbf{0.964}&\textbf{1.706}&0.841&1.521&0.837&1.485&\textbf{0.825}&\textbf{1.476}\\
&48&1.237&2.010&1.394&2.010&\textbf{1.215}&\textbf{1.937}&0.959&1.637&0.981&1.653&\textbf{0.951}&\textbf{1.624}\\
&96&1.710&2.347&1.519&2.189&\textbf{1.428}&\textbf{2.141}&1.072&1.789&1.084&1.793&\textbf{1.027}&\textbf{1.768}\\
&168&2.139&2.739&1.882&2.501&\textbf{1.303}&\textbf{2.095}&1.223&1.989&1.247&2.025&\textbf{1.139}&\textbf{1.914}\\
&336&2.444&2.965&2.632&2.972&\textbf{1.502}&\textbf{2.305}&1.222&2.083&1.279&2.127&\textbf{1.146}&\textbf{2.044}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{ETTh2} }
%&24&1.152&2.209&1.111&2.121&\textbf{1.097}&\textbf{2.126}&1.038&2.008&1.028&1.987&\textbf{1.004}&\textbf{1.965}\\
&48&1.477&2.469&1.600&2.518&\textbf{1.459}&\textbf{2.432}&1.329&2.308&1.259&2.202&\textbf{1.229}&\textbf{2.182}\\
&96&1.962&2.901&2.205&2.978&\textbf{1.869}&\textbf{2.748}&1.628&2.604&1.644&2.534&\textbf{1.570}&\textbf{2.496}\\
&168&1.898&2.919&2.128&2.991&\textbf{1.834}&\textbf{2.831}&2.148&3.021&2.062&2.903&\textbf{1.752}&\textbf{2.681}\\
&336&2.271&3.235&2.122&3.058&\textbf{2.113}&\textbf{3.003}&2.376&3.339&2.238&3.084&\textbf{1.928}&\textbf{2.847}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{ETTm2}}
%&24&0.752&1.779&0.858&1.858&\textbf{0.740}&\textbf{1.724}&0.740&1.692&0.717&1.635&\textbf{0.704}&\textbf{1.627}\\
&48&1.329&2.341&1.068&2.085&\textbf{1.034}&\textbf{2.072}&0.924&1.897&0.928&1.873&\textbf{0.894}&\textbf{1.866}\\
&96&1.261&2.283&1.274&2.255&\textbf{1.158}&\textbf{2.176}&1.085&2.010&1.046&1.985&\textbf{0.980}&\textbf{1.945}\\
&168&1.696&2.693&1.647&2.567&\textbf{1.449}&\textbf{2.469}&1.476&2.375&1.313&2.244&\textbf{1.212}&\textbf{2.162}\\
&336&2.554&3.313&3.161&3.524&\textbf{1.950}&\textbf{2.826}&1.819&2.700&1.890&2.678&\textbf{1.541}&\textbf{2.477}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{Weather}}
%&24&0.643&3.351&1.708&3.328&\textbf{0.306}&\textbf{1.429}&0.293&1.596&0.285&1.185&\textbf{0.266}&\textbf{1.149}\\
&48&0.597&2.817&1.801&3.615&\textbf{0.402}&\textbf{1.844}&0.781&2.826&0.627&2.000&\textbf{0.432}&\textbf{1.698}\\
&96&0.658&3.327&0.881&3.108&\textbf{0.285}&\textbf{1.663}&0.246&1.642&0.234&1.350&\textbf{0.223}&\textbf{1.328}\\
&168&0.398&2.260&0.379&2.036&\textbf{0.253}&\textbf{1.708}&0.192&1.392&0.187&1.240&\textbf{0.182}&\textbf{1.217}\\
&336&0.570&2.996&0.383&2.151&\textbf{0.255}&\textbf{1.712}&0.194&1.520&0.194&1.395&\textbf{0.179}&\textbf{1.311}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{CAISO}}
%&24&0.895&0.520&0.446&\textbf{0.345}&\textbf{0.408}&{0.350}&0.384&0.306&0.394&0.282&\textbf{0.322}&\textbf{0.281}\\
&48&1.789&0.740&1.596&0.635&\textbf{0.823}&\textbf{0.467}&0.599&0.384&0.614&0.360&\textbf{0.514}&\textbf{0.341}\\
&96&2.428&0.826&1.587&0.640&\textbf{1.289}&\textbf{0.576}&0.886&0.440&0.904&0.427&\textbf{0.878}&\textbf{0.428}\\
&168&2.832&0.907&2.758&0.840&\textbf{1.344}&\textbf{0.575}&1.189&0.504&1.220&0.496&\textbf{1.150}&\textbf{0.498}\\
&336&3.148&0.960&4.578&1.182&\textbf{1.809}&\textbf{0.679}&1.612&0.607&1.643&0.605&\textbf{1.518}&\textbf{0.602}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{NordPool}}
%&24&1.701&7.919&1.138&6.167&\textbf{1.007}&\textbf{5.937}&0.836&5.260&0.842&5.212&\textbf{0.833}&\textbf{5.221}\\
&48&1.632&0.765&1.628&0.750&\textbf{1.478}&\textbf{0.732}&1.190&0.639&1.266&0.650&\textbf{1.150}&\textbf{0.632}\\
&96&2.187&0.889&2.294&0.898&\textbf{2.071}&\textbf{0.852}&1.644&0.764&1.703&0.771&\textbf{1.596}&\textbf{0.756}\\
&168&2.596&0.992&2.655&0.978&\textbf{2.430}&\textbf{0.957}&2.044&0.867&2.280&0.883&\textbf{1.918}&\textbf{0.836}\\
&336&2.113&0.906&3.086&0.964&\textbf{2.079}&\textbf{0.887}&2.550&0.953&2.475&0.946&\textbf{2.098}&\textbf{0.884}\\

\midrule
\bottomrule
\end{tabular}
\begin{tablenotes}
\item $*$ means N-BEATS is re-implemented for multivariate time series forecasting; see Appendix \ref{sec:appendix_baseline} for details.
\end{tablenotes}
\end{threeparttable}
}
\vspace{-4mm}
\end{table*}


==> expfigs/tables/main_non_station_dish.tex <==

\begin{table}[!t]
% \vspace{-20mm}
\centering
\caption{Performance comparison of Dish-TS, SAN, and IN-Flow on six datasets under three seeds when taking the PatchTST as the backbone model.} \label{table:results_with_norm}
\vspace{-2mm}
\resizebox{1.0\linewidth}{!}{
\begin{threeparttable}
%\fontsize{8pt}{8}\selectfont
\small
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c}{Method}& 
\multicolumn{2}{c}{ PatchTST }&\multicolumn{2}{c}{+Dish-TS}& 
\multicolumn{2}{c}{ +SAN}&\multicolumn{2}{c}{ +IN-Flow}\\
\cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} %\cmidrule(r){11-12} 
\multicolumn{2}{c}{Metric}&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE\\
%&MSE& MAE\\
\midrule \midrule
\multirow{4}{*}{ \rotatebox{90}{ETTh1} }
& 48     & 1.128    & 1.865 & 0.975 & 1.661 & 0.971   & 1.668 & \textbf{0.936} & \textbf{1.635} \\
         & 96     & 1.320    & 2.109 & 1.100 & 1.933 & 1.093   & 1.839 & \textbf{1.025} & \textbf{1.782} \\
         & 168    & 2.001    & 2.679 & 1.229 & 2.024 & 1.110   & 1.950 & \textbf{1.077} & \textbf{1.888} \\
         & 336    & 1.784    & 2.613 & 1.352 & 2.172 & 1.251   & 2.137 & \textbf{1.121} & \textbf{2.021} \\

% \midrule
% \multirow{4}{*}{ \rotatebox{90}{ETTm2} }
% & 48     & 1.530    & 2.566 & 1.492 & 2.574 & 1.385   & 2.465 & \textbf{1.242} & \textbf{2.226} \\
%          & 96     & 2.456    & 3.469 & 1.720 & 2.766 & 1.667   & 2.603 & \textbf{1.549} & \textbf{2.507} \\
%          & 168    & 2.367    & 3.414 & 2.529 & 3.623 & 2.206   & 3.373 & \textbf{1.664} & \textbf{2.678} \\
%          & 336    & 3.313    & 4.046 & 2.623 & 3.452 & 2.478   & 3.433 & \textbf{1.893} & \textbf{2.870} \\

% \midrule
% \multirow{4}{*}{ \rotatebox{90}{ETTm2}}
% & 48     & 1.116    & 2.204 & 1.053 & 2.067 & 1.114   & 2.198 & \textbf{0.925} & \textbf{1.908} \\
%          & 96     & 1.503    & 2.699 & 1.099 & 2.072 & 1.655   & 2.423 & \textbf{0.992} & \textbf{1.965} \\
%          & 168    & 1.708    & 2.783 & 1.352 & 2.304 & 1.802   & 2.798 & \textbf{1.213} & \textbf{2.202} \\
%          & 336    & 2.482    & 3.465 & 1.657 & 2.592 & 2.083   & 3.009 & \textbf{1.564} & \textbf{2.482} \\

% \midrule
% \multirow{4}{*}{ \rotatebox{90}{Electricity}}
% &48  & 0.632 & 0.566 & 0.672 & 0.445   & 0.596 & 0.421      & \textbf{0.554} & \textbf{0.342} \\
% &96  & 0.882 & 0.698  & 0.718 & 0.434  & 0.658 & 0.379     & \textbf{0.589} & \textbf{0.341}  \\
% &168 & 1.678 & 0.541  & 1.043 & 0.512   & 0.996 & 0.454    & \textbf{0.882} & \textbf{0.389}  \\
% &336 & 2.482 & 0.814   & 2.417 & 0.833   & 2.239 & 0.781   & \textbf{2.104} & \textbf{0.768}  \\

\midrule
\multirow{4}{*}{ \rotatebox{90}{Weather}}
& 48     & 1.003    & 3.291 & 0.852 & 2.288 & 0.466   & 1.753 & \textbf{0.413} & \textbf{1.710} \\
         & 96     & 0.335    & 1.886 & 0.314 & 1.856 & 0.309   & 1.777 & \textbf{0.279} & \textbf{1.541} \\
         & 168    & 0.338    & 2.138 & 0.219 & 1.975 & 0.217   & 1.622 & \textbf{0.207} & \textbf{1.421} \\
         & 336    & 0.385    & 2.375 & 0.256 & 2.612 & 0.239   & 1.907 & \textbf{0.192} & \textbf{1.475} \\

\midrule
\multirow{4}{*}{ \rotatebox{90}{CAISO}}
& 48     & 0.986    & 0.499 & 0.838 & 0.456 & 0.748   & 0.425 & \textbf{0.641} & \textbf{0.383} \\
         & 96     & 1.098    & 0.451 & 1.216 & 0.541 & 0.901   & 0.446 & \textbf{0.828} & \textbf{0.422} \\
         & 168    & 1.369    & 0.577 & 1.396 & 0.558 & 1.216   & 0.527 & \textbf{1.161} & \textbf{0.500} \\
         & 336    & 2.541    & 0.852 & 1.925 & 0.708 & 1.831   & 0.683 & \textbf{1.636} & \textbf{0.604} \\


\midrule
\multirow{4}{*}{ \rotatebox{90}{NordPool}}
& 48     & 1.304    & 0.664 & 1.293 & 0.654 & 1.200   & 0.646 & \textbf{1.156} & \textbf{0.636} \\
         & 96     & 1.971    & 0.892 & 1.895 & 0.924 & 1.812   & 0.800 & \textbf{1.687} & \textbf{0.777} \\
         & 168    & 2.513    & 0.986 & 2.321 & 0.928 & 2.047   & 0.885 & \textbf{2.009} & \textbf{0.865} \\
         & 336    & 2.946    & 1.040 & 2.707 & 1.010 & 2.014   & 0.889 & \textbf{2.010} & \textbf{0.887} \\
\midrule
\bottomrule
\end{tabular}
\end{threeparttable}
}
\vspace{-1mm}
\end{table}



==> expfigs/tables/main_nonstaion.tex <==
% \begin{table*}[h]
% \small
% \centering
% \resizebox{\linewidth}{!}{
% \begin{threeparttable}
% \caption{Performance comparison with Non-stationary Transformers \cite{liu2022NonstatTranformers}, where Transformer/Informer/Autoformer, three backbones are coupled into Non-stationary versions (NStation-Trans/Infor/Auto) to compare
% IN-Flow-coupled versions. We report the average performance under three random seeds. Evaluations are on MSE. For the full results, please see Appendix \ref{sec:appendix_more_real_exp_results}.
% }
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
% \toprule
% Datasets & \multicolumn{3}{c}{ETTh2} & \multicolumn{3}{c}{ETTm2} & \multicolumn{3}{c}{Weather} & \multicolumn{3}{c}{CAISO}  \\
% Length & 48 & 168 & 336 & 48 & 168 & 336 & 48 & 168 & 336 & 48 & 168 & 336  \\
% \midrule
% NStation-Trans & 1.677 & 2.198 & 2.983 &0.948 & 1.587 & 2.126 & 0.551 & 0.389 & 0.323 &
% 0.850 & 1.799 & 2.282\\
% IN-Flow-Trans& \textbf{1.352} & \textbf{1.936} & \textbf{2.053} & \textbf{0.865} & \textbf{1.291} & \textbf{1.701} & \textbf{0.360}  & \textbf{0.219} & \textbf{0.210} & \textbf{0.757} & \textbf{1.245} & \textbf{1.548}\\
% \cmidrule(lr){1-13}
% Improvement & 19.4\% & 11.9\% & 31.2\% &  8.8\% & 18.7\% & 20.0\% & 
% 34.6\% & 43.7\% & 35.0\% & 10.9\% & 30.8\% & 32.1\% \\
% \midrule
% NStation-Infor & 2.094& 2.468& 2.710& 0.968& 1.697&1.987&0.566& 0.267& 0.289& 0.861& 1.406& 1.805  \\
% IN-Flow-Infor &\textbf{1.487}& \textbf{1.958}& \textbf{2.096}& \textbf{0.944}& \textbf{1.355}& \textbf{1.971}& \textbf{0.400}& \textbf{0.217}& \textbf{0.249}& \textbf{0.768}& \textbf{1.358}& \textbf{1.739}\\
% \cmidrule(lr){1-13}
% Improvement& 32.2\% & 20.7\% & 22.7\% & 2.5\% &  20.1\% & 0.8\% &  29.3\% & 18.7\% & 13.8\% &  10.8\% & 3.4\% &  3.7\%          \\
% \midrule
% NStation-Auto & 1.553& 2.007& 2.117& 1.093& 1.633& 2.166& 0.580& 0.533& 0.375& 0.844& 1.534&1.923   \\
% IN-Flow-Auto&\textbf{1.427}& \textbf{1.815}& \textbf{2.068}& \textbf{1.028}& \textbf{1.487}& \textbf{1.949}& \textbf{0.421}& \textbf{0.248}& \textbf{0.261}& \textbf{0.794}& \textbf{1.331}& \textbf{1.535}\\
% \cmidrule(lr){1-13}
% Improvement& 8.1\% & 9.6\% & 2.3\% & 5.9\% & 8.9\%  & 10.0\%  & 27.7\%   & 
%  53.4\% & 30.4\% & 5.9\%  &13.2\%  &  20.2\%           \\
% % \midrule
% % Improve & 11.3\%& 15.3\%& 21.1\%& 18.1\%& 21.4\%& 36.3\%& 
% % 17.7\%& 11.7\%& 12.3\%&
% % 29.6\%&  10.7\%&  7.7\% \\
% \bottomrule
% \end{tabular}
% \label{table:main_nonstation}
% \end{threeparttable}
% }
% \end{table*}



% \begin{table}[!h]
% \small
% % \fontsize{9.5pt}{8.6}\selectfont
% \centering
% \caption{Performance comparison with Non-stationary Transformers \cite{liu2022NonstatTranformers}, where Transformer, Informer, and Autoformer are coupled into non-stationary versions (NStation-Trans/Infor/Auto) to compare with
% IN-Flow-coupled versions. %We report the average MSE under three random seeds. 
% %See Appendix \ref{sec:appendix_more_real_exp_results} for full results.
% }
% \resizebox{\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% Datasets & \multicolumn{3}{c}{ETTh2} & \multicolumn{3}{c}{Weather} & \multicolumn{3}{c}{CAISO}  \\
% Length & 48 & 168 & 336 & 48 & 168 & 336 & 48 & 168 & 336  \\
% \midrule
% NS-Transformer & 1.677 & 2.198 & 2.983 & 0.551 & 0.389 & 0.323 &
% 0.850 & 1.799 & 2.282\\
% INF-Transformer& \textbf{1.352} & \textbf{1.936} & \textbf{2.053} &  \textbf{0.360}  & \textbf{0.219} & \textbf{0.210} & \textbf{0.757} & \textbf{1.245} & \textbf{1.548}\\
% \cmidrule(lr){1-10}
% Improvement & 19.4\% & 11.9\% & 31.2\% & 
% 34.6\% & 43.7\% & 35.0\% & 10.9\% & 30.8\% & 32.1\% \\
% \midrule
% NS-Informer & 2.094& 2.468& 2.710& 0.566& 0.267& 0.289& 0.861& 1.406& 1.805  \\
% INF-Informer &\textbf{1.487}& \textbf{1.958}& \textbf{2.096}&\textbf{0.400}& \textbf{0.217}& \textbf{0.249}& \textbf{0.768}& \textbf{1.358}& \textbf{1.739}\\
% \cmidrule(lr){1-10}
% Improvement& 32.2\% & 20.7\% & 22.7\% &  29.3\% & 18.7\% & 13.8\% &  10.8\% & 3.4\% &  3.7\%          \\
% \midrule
% NS-Autoformer & 1.553& 2.007& 2.117&  0.580& 0.533& 0.375& 0.844& 1.534&1.923   \\
% INF-Autoformer&\textbf{1.427}& \textbf{1.815}& \textbf{2.068}& \textbf{0.421}& \textbf{0.248}& \textbf{0.261}& \textbf{0.794}& \textbf{1.331}& \textbf{1.535}\\
% \cmidrule(lr){1-10}
% Improvement& 8.1\% & 9.6\% & 2.3\%  & 27.7\%   & 
%  53.4\% & 30.4\% & 5.9\%  &13.2\%  &  20.2\%           \\
% % \midrule
% % Improve & 11.3\%& 15.3\%& 21.1\%& 18.1\%& 21.4\%& 36.3\%& 
% % 17.7\%& 11.7\%& 12.3\%&
% % 29.6\%&  10.7\%&  7.7\% \\
% \bottomrule
% \end{tabular}
% \label{table:main_nonstation}
% \end{threeparttable}
% }
% % \vspace{-2mm}
% \end{table}






\begin{table}[!h]
\small
% \fontsize{9.5pt}{8.6}\selectfont
\centering
\caption{Performance comparison with non-stationary transformers, where Transformer, Informer, and Autoformer are coupled into non-stationary versions to compare with
IN-Flow-coupled versions. %We report the average MSE under three random seeds. 
%See Appendix \ref{sec:appendix_more_real_exp_results} for full results.
} \label{table:main_nonstation}
\vspace{-2mm}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{l|cc|cc|cc}
\toprule
Datasets & \multicolumn{2}{c}{ETTm2} & \multicolumn{2}{c}{Weather} & \multicolumn{2}{c}{CAISO}  \\
Length & 48  & 336 & 48  & 336 & 48 & 336  \\
\midrule
NS-Transformer & 1.677  & 2.983 & 0.551  & 0.323 &
0.850  & 2.282\\
INF-Transformer& \textbf{1.352} & \textbf{2.053} &  \textbf{0.360}   & \textbf{0.210} & \textbf{0.757}  & \textbf{1.548}\\
\cmidrule(lr){1-7}
Improvement & 19.4\%  & 31.2\% & 
34.6\% &   35.0\% & 10.9\%  & 32.1\% \\
\midrule
NS-Informer & 2.094 & 2.710& 0.566&  0.289& 0.861&  1.805  \\
INF-Informer &\textbf{1.487}& \textbf{2.096}&\textbf{0.400}& \textbf{0.249}& \textbf{0.768}&  \textbf{1.739}\\
\cmidrule(lr){1-7}
Improvement& 32.2\%  & 22.7\% &  29.3\%  & 13.8\% &   3.4\% &  3.7\%          \\
\midrule
NS-Autoformer & 1.553&  2.117& 0.580&  0.375& 0.844& 1.923   \\
INF-Autoformer&\textbf{1.427}&  \textbf{2.068}& \textbf{0.421}&  \textbf{0.261}& \textbf{0.794}&\textbf{1.535}\\
\cmidrule(lr){1-7}
Improvement& 8.1\%  & 2.3\%  & 27.7\%   & 
  30.4\% & 5.9\%    &  20.2\%           \\
% \midrule
% Improve & 11.3\%& 15.3\%& 21.1\%& 18.1\%& 21.4\%& 36.3\%& 
% 17.7\%& 11.7\%& 12.3\%&
% 29.6\%&  10.7\%&  7.7\% \\
\bottomrule
\end{tabular}
\end{threeparttable}
}
\vspace{-1mm}
\end{table}

==> tables/main_ablation.tex <==

\begin{wraptable}{r}{0.65\linewidth}
% \begin{table}[h]
\small
\centering
% \begin{threeparttable}
\vspace{-6mm}
\caption{Ablation studies with taking N-BEATS as the backbone. Evaluations are the average performance of four seeds on MSE. Underlined are the best results. See Appendix \ref{sec:appendix_ablation_exp_results} for full results.
} \label{table:main_brief_ablation}
% \resizebox{\linewidth}{!}{
\begin{tabular}{p{0.01cm} c|ccccc}
\toprule
&& {\scriptsize RealNVP} & {\scriptsize RealNVP-c} & {\scriptsize IN-Flow-J} & {\scriptsize IN-Flow-T} & {\scriptsize IN-Flow} \\
%&& { RealNVP-c} & { RealNVP} & { IN-Flow-J} & { IN-Flow-T} & { IN-Flow} \\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize ETTh2} }
&{\scriptsize 48}&13.823&1.380&1.264&1.240& \underline{1.229}\\
&{\scriptsize 168}&13.493&2.192&1.848&1.772&\underline{1.752}\\
&{\scriptsize 336}&11.690&2.317&\underline{1.872}&1.961&{1.928}\\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize ETTm2} }
&{\scriptsize 48}&12.291&1.031&\underline{0.876}&0.938&{0.894}\\
&{\scriptsize 168}&14.474&1.530&1.231&1.214&\underline{1.212}\\
&{\scriptsize 336}&16.525&1.826&1.546&1.567&\underline{1.541}\\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize Weather} }
&{\scriptsize 48}&1.039&0.533&0.495&0.460&\underline{0.432}\\
&{\scriptsize 168}&0.771&0.183&0.186&0.191&\underline{0.182}\\
&{\scriptsize 336}&0.604&0.190&0.183&0.193&\underline{0.179}\\
\midrule
\multirow{3}{*}{ \rotatebox{90}{\scriptsize CAISO} }
&{\scriptsize 48}&4.355&0.568&0.541&0.516&\underline{0.514}\\
&{\scriptsize 168}&5.013&{1.126}&\underline{1.054}&1.153&1.150\\
&{\scriptsize 336}&3.710&1.479&\underline{1.358}&1.535&1.518\\
\bottomrule
\end{tabular}
% }
% \end{table}
\end{wraptable}




==> tables/main_exp_old.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{threeparttable}
% \fontsize{8.5pt}{9}\selectfont
\small
\caption{Performance comparison of time series forecasting on backbone models (Autoformer and N-BEATS) with z-score-norm, RevIN and IN-Flow. The length of windows is prolonged from 48 to 336 to cover short/long-term forecasting. %The reported metrics are the average results under four seeds (see Appendix \ref{sec:appendix_more_real_evaluation_details}).
%Due to space limit, results of Informer are in Appendix.
} \label{table:main_exp}
\begin{tabular}{c|c|cccccc|cccccc}
\toprule
\multicolumn{2}{c}{Method}& \multicolumn{2}{c}{Autoformer}&\multicolumn{2}{c}{+{RevIN}}& \multicolumn{2}{c|}{+IN-Flow}&\multicolumn{2}{c}{{N-BEATS{$^*$}}}& 
\multicolumn{2}{c}{+{RevIN}}&   \multicolumn{2}{c}{+{IN-Flow}}\\ 
\cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14} 
\multicolumn{2}{c}{Metric}&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE&
MSE& MAE&  MSE& MAE\\
\midrule \midrule
\multirow{4}{*}{ \rotatebox{90}{ETTh1} }
%&24&0.988&1.774&1.161&1.846&\textbf{0.964}&\textbf{1.706}&0.841&1.521&0.837&1.485&\textbf{0.825}&\textbf{1.476}\\
&48&1.237&2.010&1.394&2.010&\textbf{1.215}&\textbf{1.937}&0.959&1.637&0.981&1.653&\textbf{0.951}&\textbf{1.624}\\
&96&1.710&2.347&1.519&2.189&\textbf{1.428}&\textbf{2.141}&1.072&1.789&1.084&1.793&\textbf{1.027}&\textbf{1.768}\\
&168&2.139&2.739&1.882&2.501&\textbf{1.303}&\textbf{2.095}&1.223&1.989&1.247&2.025&\textbf{1.139}&\textbf{1.914}\\
&336&2.444&2.965&2.632&2.972&\textbf{1.502}&\textbf{2.305}&1.222&2.083&1.279&2.127&\textbf{1.146}&\textbf{2.044}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{ETTh2} }
%&24&1.152&2.209&1.111&2.121&\textbf{1.097}&\textbf{2.126}&1.038&2.008&1.028&1.987&\textbf{1.004}&\textbf{1.965}\\
&48&1.477&2.469&1.600&2.518&\textbf{1.459}&\textbf{2.432}&1.329&2.308&1.259&2.202&\textbf{1.229}&\textbf{2.182}\\
&96&1.962&2.901&2.205&2.978&\textbf{1.869}&\textbf{2.748}&1.628&2.604&1.644&2.534&\textbf{1.570}&\textbf{2.496}\\
&168&1.898&2.919&2.128&2.991&\textbf{1.834}&\textbf{2.831}&2.148&3.021&2.062&2.903&\textbf{1.752}&\textbf{2.681}\\
&336&2.271&3.235&2.122&3.058&\textbf{2.113}&\textbf{3.003}&2.376&3.339&2.238&3.084&\textbf{1.928}&\textbf{2.847}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{ETTm2}}
%&24&0.752&1.779&0.858&1.858&\textbf{0.740}&\textbf{1.724}&0.740&1.692&0.717&1.635&\textbf{0.704}&\textbf{1.627}\\
&48&1.329&2.341&1.068&2.085&\textbf{1.034}&\textbf{2.072}&0.924&1.897&0.928&1.873&\textbf{0.894}&\textbf{1.866}\\
&96&1.261&2.283&1.274&2.255&\textbf{1.158}&\textbf{2.176}&1.085&2.010&1.046&1.985&\textbf{0.980}&\textbf{1.945}\\
&168&1.696&2.693&1.647&2.567&\textbf{1.449}&\textbf{2.469}&1.476&2.375&1.313&2.244&\textbf{1.212}&\textbf{2.162}\\
&336&2.554&3.313&3.161&3.524&\textbf{1.950}&\textbf{2.826}&1.819&2.700&1.890&2.678&\textbf{1.541}&\textbf{2.477}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{Weather}}
%&24&0.643&3.351&1.708&3.328&\textbf{0.306}&\textbf{1.429}&0.293&1.596&0.285&1.185&\textbf{0.266}&\textbf{1.149}\\
&48&0.597&2.817&1.801&3.615&\textbf{0.402}&\textbf{1.844}&0.781&2.826&0.627&2.000&\textbf{0.432}&\textbf{1.698}\\
&96&0.658&3.327&0.881&3.108&\textbf{0.285}&\textbf{1.663}&0.246&1.642&0.234&1.350&\textbf{0.223}&\textbf{1.328}\\
&168&0.398&2.260&0.379&2.036&\textbf{0.253}&\textbf{1.708}&0.192&1.392&0.187&1.240&\textbf{0.182}&\textbf{1.217}\\
&336&0.570&2.996&0.383&2.151&\textbf{0.255}&\textbf{1.712}&0.194&1.520&0.194&1.395&\textbf{0.179}&\textbf{1.311}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{CAISO}}
%&24&0.895&0.520&0.446&\textbf{0.345}&\textbf{0.408}&{0.350}&0.384&0.306&0.394&0.282&\textbf{0.322}&\textbf{0.281}\\
&48&1.789&0.740&1.596&0.635&\textbf{0.823}&\textbf{0.467}&0.599&0.384&0.614&0.360&\textbf{0.514}&\textbf{0.341}\\
&96&2.428&0.826&1.587&0.640&\textbf{1.289}&\textbf{0.576}&0.886&0.440&0.904&0.427&\textbf{0.878}&\textbf{0.428}\\
&168&2.832&0.907&2.758&0.840&\textbf{1.344}&\textbf{0.575}&1.189&0.504&1.220&0.496&\textbf{1.150}&\textbf{0.498}\\
&336&3.148&0.960&4.578&1.182&\textbf{1.809}&\textbf{0.679}&1.612&0.607&1.643&0.605&\textbf{1.518}&\textbf{0.602}\\
\midrule
\multirow{4}{*}{ \rotatebox{90}{NordPool}}
%&24&1.701&7.919&1.138&6.167&\textbf{1.007}&\textbf{5.937}&0.836&5.260&0.842&5.212&\textbf{0.833}&\textbf{5.221}\\
&48&1.632&0.765&1.628&0.750&\textbf{1.478}&\textbf{0.732}&1.190&0.639&1.266&0.650&\textbf{1.150}&\textbf{0.632}\\
&96&2.187&0.889&2.294&0.898&\textbf{2.071}&\textbf{0.852}&1.644&0.764&1.703&0.771&\textbf{1.596}&\textbf{0.756}\\
&168&2.596&0.992&2.655&0.978&\textbf{2.430}&\textbf{0.957}&2.044&0.867&2.280&0.883&\textbf{1.918}&\textbf{0.836}\\
&336&2.113&0.906&3.086&0.964&\textbf{2.079}&\textbf{0.887}&2.550&0.953&2.475&0.946&\textbf{2.098}&\textbf{0.884}\\

\midrule
\bottomrule
\end{tabular}
\begin{tablenotes}
\item $*$ means N-BEATS is re-implemented for multivariate time series forecasting; see Appendix \ref{sec:appendix_baseline} for details.
\end{tablenotes}
\end{threeparttable}
}
\vspace{-4mm}
\end{table*}

